Semantic Mapping with Simultaneous Object Detection and Localization

We present a filtering-based method for semantic mapping to simultaneously detect objects and localize their 6 degree-of-freedom pose. For our method, called Contextual Temporal Mapping (or CT-Map), we represent the semantic map as a belief over object classes and poses across an observed scene. Inference for the semantic mapping problem is then modeled in the form of a Conditional Random Field (CRF). CT-Map is a CRF that considers two forms of relationship potentials to account for contextual relations between objects and temporal consistency of object poses, as well as a measurement potential on observations. A particle filtering algorithm is then proposed to perform inference in the CT-Map model. We demonstrate the efficacy of the CT-Map method with a Michigan Progress Fetch robot equipped with a RGB-D sensor. Our results demonstrate that the particle filtering based inference of CT-Map provides improved object detection and pose estimation with respect to baseline methods that treat observations as independent samples of a scene.

==> motivating_scenario.tex <==
\section{Motivating Scenario}
Domestic environment is highly dynamic in a way that most objects have varying locations from time to time except for furnitures and appliances. A service robot should be able to efficiently search and localize objects of interest in the highly dynamic environment. As the robot gained more observations of the environment over time, it can start to build up knowledge on probable locations where various objects can be, which helps the robot to efficiently search for particular objects that are needed for user commanded tasks. 

For example, when a person orders cereal for breakfast, the robot needs to search and gather a bowl, bottled milk and boxed cereal, where each of them is probably but no necessarily located in the kitchen cabinet, fridge and on the kitchen counter respectively. Based on its past observations, the robot needs to reason over places to search for these objects, ranked by the probability of the objects occurrences.

==> old_modeling.tex <==
\section{Old Modeling}
We apply sequential bayesian filtering to estimate the belief over objects $O$ given the robot poses and observations,
\[ p(O_t|x_{1:t}, z_{1:t}) = \prod_{i=1}^N p(o^i_t|x_{1:t}, z_{1:t}) \]
we assume the distributions over different objects are independent from each other. The belief of each object $o^i$ is updated through bayesian filtering,
\begin{equation}
\begin{split}
p(o^i_t|x_{1:t}, z_{1:t}) 
\propto & p(z_t|o^i_t, x_{1:t},z_{1:t-1}) p(o^i_t|x_{1:t},z_{1:t-1}) \\
\propto & \underbrace{p(z_t|o^i_t,x_t)}_{likelihood} \underbrace{p(o^i_t|x_{1:t-1},z_{1:t-1})}_{prediction}
\end{split}
\end{equation}
The \textit{prediction} term can be further expanded following the law of total probability,
\begin{equation}
\begin{split}
p(o^i_t|x_{1:t-1},z_{1:t-1}) \propto & \int_{o^i_{t-1}} \int_{u^i_{t-1}} p(o^i_t|o^i_{t-1}, u^i_{t-1}) \\
& p(o^i_{t-1}, u^i_{t-1}|x_{1:t-1}, z_{1:t-1})du^i_{t-1}do^i_{t-1} \\
\propto & \int_{o^i_{t-1}} \int_{u^i_{t-1}} p(o^i_t|o^i_{t-1}, u^i_{t-1}) \\
& p(u^i_{t-1})p(o^i_{t-1}|x_{1:t-1}, z_{1:t-1})du^i_{t-1}do^i_{t-1}
\end{split}
\end{equation}
The action $u^i_{t-1}$ applied on the object is independent from robot trajectory $x_{1:t-1}$ and observation history $z_{1:t-1}$.

\subsection{Action Modeling}
We model the action $u$ in both \textit{continuous} and \textit{discrete} space. \textbf{\textit{Continuous Action}}: when the object is within the field of view, we model $u$ as a continuous random variable that follows Gaussian distribution with zero mean and small variance, such that $u$ leads to prediction of small object movements in 3D,
\[ o^i_t \sim \mathcal{N}(o^i_{t-1}, \, \sigma^{2}) \]
 \textbf{\textit{Discrete Action}}: when the object is out of the field of view, we model $u$ as a discrete random variable that follows certain distribution $p(u)$ on a set of high-level actions $\{stay, place\_on(o^c), place\_in(o^c)\}$, denoting that object has not been moved onto/into other objects, and moved and placed on or into object with class label $o^c$ respectively. For example, if a Pringle bottle was last seen on a rack, but other Pringle bottles have been observed to be $place\_on(table)$ in the past, then the robot should be able to predict that the Pringle bottle can be moved and placed on a table after not seeing it for a while. Thus discrete actions capture contextual relations between objects.
 
In our experiments, for each object class, $p(u)$ starts as an uniform distribution. Given converged estimates of object poses, inter-object relations $(on, in)$ can be derived using some heuristics. $p(u)$ is incrementally updated based on these inter-object relations through running average. 

\color{gray}
TODO: 
\begin{itemize}
\item
elaborate on how to determine whether the object is in view or not, such that it is clear when the action will switch from continuous to discrete, and vice versa
\item
elaborate on how $p(o^i_t|o^i_{t-1}, u^i_{t-1})$ looks like for discrete actions
\end{itemize}

\color{black}

% i.e., $u^i \sim \mathcal{N}(\mu, \, \sigma^{2})$.
%Steps in the equation above are derived based on 1) Bayesian Theorem, 2) conditional independence between $z_t$ and $(z_{1:t-1}, x_{1:t-1})$ given $(o^i_t, x_t)$, 3) law of total probability, 4) action $u^i_{t-1}$ applied on the object is independent from robot trajectory $x_{1:t-1}$ and observation history $z_{1:t-1}$.

==> problem_statement.tex <==
\section{Problem Statement}
To perform object search and execute mobile manipulation tasks in the human environment, the robot needs to understand its surroundings by localizing various objects while visiting different places, and maintain a belief over objects locations for efficient object search.
